An Experience Report on Machine Learning Reproducibility: Guidance for Practitioners and TensorFlow Model Garden Contributors

Machine learning techniques are becoming a fundamental tool for scientific and engineering progress. These techniques are applied in contexts as diverse as astronomy and spam filtering. However, correctly applying these techniques requires careful engineering. Much attention has been paid to the technical potential; relatively little attention has been paid to the software engineering process required to bring research-based machine learning techniques into practical utility. Technology companies have supported the engineering community through machine learning frameworks such as TensorFLow and PyTorch, but the details of how to engineer complex machine learning models in these frameworks have remained hidden. To promote best practices within the engineering community, academic institutions and Google have partnered to launch a Special Interest Group on Machine Learning Models (SIGMODELS) whose goal is to develop exemplary implementations of prominent machine learning models in community locations such as the TensorFlow Model Garden (TFMG). The purpose of this report is to define a process for reproducing a state-of-the-art machine learning model at a level of quality suitable for inclusion in the TFMG. We define the engineering process and elaborate on each step, from paper analysis to model release. We report on our experiences implementing the YOLO model family with a team of 26 student researchers, share the tools we developed, and describe the lessons we learned along the way.

==> extras/glossary.tex <==
\usepackage[utf8]{inputenc}
\usepackage{glossaries}

\makeglossaries

\newglossaryentry{hyperparameter}{
  name={hyperparameter},
  description={Parameters that define the model architecture and training process.}
}

\newglossaryentry{TFMG}{
  name={TFMG},
  description={TensorFlow Model Garden}
}

==> extras/yolo-folders.tex <==
\definecolor{folderbg}{RGB}{124,166,198}
\definecolor{folderborder}{RGB}{110,144,169}

\def\Size{4pt}
\tikzset{
  folder/.pic={
    \filldraw[draw=folderborder,top color=folderbg!50,bottom color=folderbg]
      (-1.05*\Size,0.2\Size+5pt) rectangle ++(.75*\Size,-0.2\Size-5pt);  
    \filldraw[draw=folderborder,top color=folderbg!50,bottom color=folderbg]
      (-1.15*\Size,-\Size) rectangle (1.15*\Size,\Size);
  }
}

\begin{forest}
  for tree={
    font=\ttfamily,
    grow'=0,
    child anchor=west,
    parent anchor=south,
    anchor=west,
    calign=first,
    inner xsep=7pt,
    edge path={
      \noexpand\path [draw, \forestoption{edge}]
      (!u.south west) +(7.5pt,0) |- (.child anchor) pic {folder} \forestoption{edge label};
    },
    before typesetting nodes={
      if n=1
        {insert before={[,phantom]}}
        {}
    },
    fit=band,
    before computing xy={l=15pt},
  }  
[yolo
  [common
  ]
  [configs
  ]
  [dataloaders
  ]
  [demos
  ]
  [losses
  ]
  [modeling
  ]
  [ops
  ]
  [tasks
  ]
  [utils
  ]
]
\end{forest}

==> figures/folder-table.tex <==
\begin{tabular}{|l|l|l|}
\hline
  \textbf{Folder} & \textbf{Required} &        \textbf{Description}                                      \\ \hline
dataloaders & Yes        & \begin{tabular}[c]{@{}l@{}}Decoders and parsers for \\ your data pipeline.\end{tabular}                                                                                                       \\ \hline
modeling    & Yes        & \begin{tabular}[c]{@{}l@{}}Model and the building \\ blocks.\end{tabular}                      \\ \hline
losses      & Yes        & \begin{tabular}[c]{@{}l@{}}Loss function.\end{tabular}                                               \\ \hline \hline
common      & Yes        & \begin{tabular}[c]{@{}l@{}}Necessary registry imports. \\ The tasks and configs need to be \\ registered before execution.\end{tabular}                                                    \\ \hline
configs     & Yes        & \begin{tabular}[c]{@{}l@{}}Necessary \emph{config} files for \\ the task class to train and evaluate \\ the model.\end{tabular}                                                     
\\ \hline
ops         & Yes        & \begin{tabular}[c]{@{}l@{}}Necessary utility \\ functions used by the data \\ pipeline, loss function and \\ modeling.\end{tabular}                                                  \\ \hline
tasks       & Yes        & \begin{tabular}[c]{@{}l@{}}Tasks for running the \\ model. Tasks are essentially the \\ main driver for training and \\ evaluating the model.\end{tabular}                                  \\ \hline \hline
utils       & No       & \begin{tabular}[c]{@{}l@{}}Other utility functions \\ downloading weights from the \\ original model’s repository, datasets \\ from external sources, and the test \\ cases for these functions.\end{tabular} \\ \hline
demos       & No       & \begin{tabular}[c]{@{}l@{}}Files needed to create a \\ Jupyter Notebook/Google Colab \\ demo of the model.\end{tabular}                                                        \\ \hline
\end{tabular}

==> figures/paper-analysis-old.tex <==
\begin{tabular}{|c|c|l|l|}
\hline
\textbf{Category}& \textbf{Component} & \multicolumn{1}{c|}{\textbf{Description}} & \multicolumn{1}{c|}{\textbf{YOLO v3}} \\ \hline
\multirow{4}{*}{\textit{Overview}} & 
\textit{\begin{tabular}[c]{@{}c@{}}
Model\\ Purpose\end{tabular}} &
\begin{tabular}[c]{@{}l@{}}
The model development approach depends on the type of \\
model being implemented and its primary function. Deep\\
Learning code performs a variety of tasks. Typical\\
examples are object detection (OD) and natural\\
language processing (NLP).
\end{tabular}                                                                                                                                                    &
\begin{tabular}[c]{@{}l@{}}
Detect Objects\\
Classify Objects
\end{tabular} \\ \cline{2-4} 
& \textit{\begin{tabular}[c]{@{}c@{}}Code \\ Availability\end{tabular}} 
&
\begin{tabular}[c]{@{}l@{}}
The existence of an official or accurate unofficial\\
implementation can serve as a reference during the model\\
engineering process.\end{tabular} & 
\begin{tabular}[c]{@{}l@{}}
Original Darknet\\ 
Repository\end{tabular}  
\\ \cline{2-4} 
& \textit{\begin{tabular}[c]{@{}c@{}}Library \\ Used\end{tabular}}                & \begin{tabular}[c]{@{}l@{}}Deep Learning can be complicated and functions will vary\\ based on the programming language and the \textbackslash{}ML library\\ used. Knowing what library the algorithm's source code\\ uses will help, because certain operations will directly\\ translate to \TF API functions, whereas others\\will require\\ custom operations.\end{tabular}          & Darknet C Library \\ \cline{2-4} & 
\textit{\begin{tabular}[c]{@{}c@{}}Network \\ Referenced\end{tabular}} & \begin{tabular}[c]{@{}l@{}}If there are other neural networks referenced, it will useful\\for future\\ reference to refer to its source code while reconstructing the\\ model.\end{tabular}             & 
\begin{tabular}[c]{@{}l@{}}ResNet\\ YOLO v2\\ Faster RCNN\\ RetinaNet\end{tabular}                               \\ \hline
\multirow{6}{*}{\textit{\begin{tabular}[c]{@{}c@{}}Model \&\\ Design\end{tabular}}}         & \textit{\begin{tabular}[c]{@{}c@{}}Model\\  Architecture\end{tabular}}          & \begin{tabular}[c]{@{}l@{}}The model cannot be built without knowing its\\ architecture,  i.e the type, size and connection of layers.\end{tabular}                                                                                                                                                                                                                                                                                                      & Architecture provided                                                                                                                                   \\ \cline{2-4} 
                                                                                            & \textit{\begin{tabular}[c]{@{}c@{}}Model \\ Sub-Networks\end{tabular}}          & \begin{tabular}[c]{@{}l@{}}Sub-networks are defined structures such as a backbone or\\ decoder, that can be built independently because they serve a\\ specific purpose. These elements can be built in parallel\\ during the model engineering process.\end{tabular}                                                                                                                                                                                          & \begin{tabular}[c]{@{}l@{}}Backbone \\ Classification Head\end{tabular}                                                                    \\ \cline{2-4} 
                                                                                            & \textit{\begin{tabular}[c]{@{}c@{}}Model Building \\ Blocks\end{tabular}}       & \begin{tabular}[c]{@{}l@{}}Building blocks are a set of layers or components that are\\ repeatedly seen in a particular order within the model\\ architecture. Having well-defined building blocks will ensure\\ components is being reused whenever possible, with no\\ redundant code segments.\end{tabular}                                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}DarkResNet Block\\ Routing Layers\\ DetectionRouteProcessing\\ DarkBlock\end{tabular} \\ \cline{2-4} 
                                                                                            & \textit{Custom Layers}                                                          & \begin{tabular}[c]{@{}l@{}}TensorFlow has predefined layers, but most Machine\\ Learning models will require custom layers that perform a\\ specific function. Once a custom layer is built, it can be used\\ anywhere within the Model Garden.\end{tabular}                                                                                                                                                                                                   & DarkConv                                                                                                                                                \\ \cline{2-4} 
                                                                                            & \textit{Loss Functions}                                                         & \begin{tabular}[c]{@{}l@{}}The objective of a Machine Learning model is to adjust\\ parameters such that the loss function has reached its global\\ minimum. Loss functions are often complicated and require\\ numerous operations.\end{tabular}                                                                                                                                                                                                              & Equation provided                                                                                                                                       \\ \cline{2-4} 
                                                                                            & \textit{Output Structure}                                                       & \begin{tabular}[c]{@{}l@{}}Knowing the final output structure will help during the unit and \\ differential testing phases of model development.\end{tabular}                                                                                                                                                                                                                                                                                                  & Architecture provided                                                                                                                                   \\ \hline
\multirow{5}{*}{\textit{\begin{tabular}[c]{@{}c@{}}Training \& \\ Evaluation\end{tabular}}} & \textit{Dataset Used}                                                           & \begin{tabular}[c]{@{}l@{}}Without using the same dataset as the research paper, it is \\ not possible to reproduce the results obtained in the original\\ implementation. Most State-Of-The-Art models use well-known\\ datasets, which are usually large in size and relatively easy to\\ find and download.\end{tabular}                                                                                                                                    & COCO                                                                                                                                                    \\ \cline{2-4} 
                                                                                            & \textit{\begin{tabular}[c]{@{}c@{}}Pre-processing \\ Functions\end{tabular}}    & \begin{tabular}[c]{@{}l@{}}Pre-processing functions are used to format \\ and augment the dataset before feeding input to the model.\end{tabular}                                                                                                                                                                                                                                                                                                           & \begin{tabular}[c]{@{}l@{}}Random jitter\\ Random crop\\ Random zoom\\ Provided in repository\end{tabular}       \\ \cline{2-4} 
                                                                                            & \textit{\begin{tabular}[c]{@{}c@{}}Output Processing \\ Functions\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Once the model has processed the input, the output may need\\ to be adjusted and modified appropriately.\end{tabular}                                                                                                                                                                                                                                                                                                               & None                                                                                                                                                    \\ \cline{2-4} 
                                                                                            & \textit{\begin{tabular}[c]{@{}c@{}}Testing \& Target\\ Metrics\end{tabular}}    & \begin{tabular}[c]{@{}l@{}}Testing Metrics are metrics used to evaluate a machine\\ learning model. Some metrics are built into TensorFlow. \\ Others must be custom-made. Target Metrics \\ are the metric values obtained in the original implementation,\\ and will be provided in the research paper. The closer the \\ exemplar's performance metrics are to the original one,\\ the more accurate the exemplar is.\end{tabular} & \begin{tabular}[c]{@{}l@{}}$AP_{50}$\\ $AP_{75}$\\ $AP_S$\\ $AP_M$\\ $AP_L$\end{tabular}  \\ \cline{2-4} 
                                                                                            & \textit{Training Steps}                                                         & \begin{tabular}[c]{@{}l@{}}A model may have special steps to follow during the training process.\end{tabular}                                                                                                                                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}Training schedule\\ Input specifications\end{tabular}                                                           \\ \hline
\end{tabular}

==> figures/yolo-paper-table.tex <==
\begin{tabular}{|l|l|}
\hline
Paper Aspect & YOLO v3 \\ \hline
Model Purpose & \begin{tabular}[c]{@{}l@{}}Detect and Classify \\ Objects\end{tabular}                                               \\ \hline
Code Availability & Darknet: GitHub \\ \hline
Library Used & Darknet C Library \\ \hline
Network Referenced & 
\begin{tabular}[c]{@{}l@{}}
ResNet, YOLO v2,
\\ Faster RCNN,
\\ RetinaNet
\end{tabular} \\ \hline
Model Architecture & Provided \\ \hline
Model Sub-Networks & 
\begin{tabular}[c]{@{}l@{}}
Backbone - Classification
\\ Head
\end{tabular} \\ \hline
Model Building Blocks & 
\begin{tabular}[c]{@{}l@{}}
DarkResNet Block,\\ 
Routing Layers,\\ 
DetectionRouteProcessing, \\
DarkBlock\end{tabular} \\ \hline
Custom Layers & DarkConv \\ \hline
Loss Functions & Equation given \\ \hline
Output Structure & Provided in architecture \\ \hline
Dataset Used & COCO \\ \hline
Image Pre-processing & Provided in paper \\ \hline
Output Processing & Provided in paper \\ \hline
Testing Metrics \& Callback & mAP, AP50\\ \hline
Testing Steps &  \\ \hline
Target Metrics  &  \\ \hline
\end{tabular}

